Clover: Toward Sustainable AI with Carbon-Aware Machine Learning Inference Service

This paper presents a solution to the challenge of mitigating carbon emissions from hosting large-scale machine learning (ML) inference services. ML inference is critical to modern technology products, but it is also a significant contributor to carbon footprint. We introduce Clover, a carbon-friendly ML inference service runtime system that balances performance, accuracy, and carbon emissions through mixed-quality models and GPU resource partitioning. Our experimental results demonstrate that Clover is effective in substantially reducing carbon emissions while maintaining high accuracy and meeting service level agreement (SLA) targets.

==> sections/old_motivation.tex <==
% \section{Motivation}
% \label{sec:motiv}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.48]{figures/motiv1_variant.pdf}    
%     \hrule
%     \vspace{-0.4cm}    
%     \caption{Using mixed-quality models provides an opportunity to reduce carbon footprint of model serving significantly while maintaining high accuracy.}
%     \vspace{-0.5cm}
%     \label{fig:motiv1_variant}
% \end{figure}

% In this section, we provide three key insights that motivate the design of or \sol{} inference system. 

% \vspace{1.5mm}
% \noindent\textbf{Opportunity 1. Creating a mix of model variants (i.e., mix of low- and high-quality models) provides an opportunity for a significant reduction in the carbon footprint, while minimal loss in the overall average accuracy.} 

% \vspace{1.5mm}

% Fig.~\ref{fig:motiv1_variant} shows a plot of accuracy vs. carbon savings for mixed-quality inference services hosted on a 4-GPU system. The x-axis representing the carbon footprint reduction and the y-axis representing the average inference accuracy of different combinations of model variants(more methodology details available in Sec.~\ref{sec:method}). Recall that different model variants can offer different levels of accuracy, and their corresponding carbon footprint also varies. A model that offers higher accuracy is likely to be more complex and more computationally-intensive -- leading to higher operational energy and carbon footprint. 

% The accuracy and carbon emission are relative to the default configuration where we host the highest-quality model variant on all GPUs, represented by the star point (0,1). For fair evaluation, while calculating the carbon emission/footprint savings, we have kept the carbon intensity the same (i.e., the greenness of the energy source powering the infrastructure is the same across all points). 

% Fig.~\ref{fig:motiv1_variant} reveals the trade-off between accuracy and carbon footprint reduction. For example, a combination of high-quality and low-quality models can provide over 60\% carbon footprint savings, while incurring less than 10\% accuracy degradation compared to the highest-quality model. As expected, the opportunity for carbon savings increases with higher tolerance for accuracy degradation (more than 80\% carbon savings for 10\% accuracy loss). 

% Although, it is not visually depicted, determining the combination of models with different accuracy-quality to attain a give accuracy degradation is not trivial. This is because multiple models with different quality may provide different carbon savings.  This problem becomes more challenging in \sol{}'s case because \sol{}'s needs to dynamically respond to the varying carbon intensity of the energy source (e.g., the fraction of energy coming from renewable sources may vary over the day). 

% Next, we discuss the third aspect of the design trade-off -- latency of the ML inference queries. In particular, we show that co-location of inference service can reduce carbon footprint, but increase the latency (carbon footprint savings vs. latency trade-offs). 


% \begin{figure}
%     \centering
%     \includegraphics[scale=0.46]{figures/motiv2_mig.pdf}    
%     \hrule
%     \vspace{-0.4cm}    
%     \caption{MIG GPU partitioning enables the opportunity to reduce carbon footprint of modeling serving because it allows better resource utilization. However, partitioning leads to latency degradation -- presenting a trade-off between carbon emission and performance. C1 is full GPU, C2 partitions the GPU into \{\texttt{4g}, \texttt{2g}, \texttt{1g}\} and C3 partitions the GPU into seven \texttt{1g} slices.}
%     %For simplicity, the same model is used across all three partitions to avoid accuracy trade-offs. 
%     \vspace{-0.5cm}
%     \label{fig:motiv2_mig}
% \end{figure}

% \vspace{1.5mm}
% \noindent\textbf{Opportunity 2. Partitioning a GPU hardware provides an opportunity to reduce the carbon footprint because it allows more efficient usage of GPU resources. However, co-location leads to higher latency (i.e., higher SLA violation rate) -- making it challenging to exploit this opportunity space.} 

% \vspace{1.5mm}

% Fig.~\ref{fig:motiv2_mig} shows the effects of partitioning the GPU on the carbon footprint and the inference latency. Before drawing observations from this experiment, we briefly describe the setup. 

% The GPU is configured to C1, C2, C3, representing the MIG configurations 1, 3, and 19, respectively in Fig.~\ref{fig:bkgd1_mig}. We have hosted the same model variant (i.e., the model quality is fixed) across all partitions of the GPU and each partition hosts one instance of the inference service.  We keep the model quality the same to avoid complexities arising from accuracy trade-offs in this experiment -- which was focus of the previous observation. For consistency, we kept the carbon intensity the same throughout the experiment. 

% Fig.~\ref{fig:motiv2_mig} shows that when the GPU goes from an non-partitioned state (i.e., $C1$) to a fine-grained partitioned state ($C3$), we can reduce the carbon footprint by 30\% when serving the same number of inference requests. This is because fine-grained partitioning allows higher degree of co-location, and hence, better resource utilization. This leads to lower carbon emission per query. 

% All resources of a large, non-partitioned GPU can not be fully utilized by a single hosted model. Increasing co-location of model allows better resource utilization and hence, lower energy consumption (carbon footprint) per query on an average. But, as expected, co-location of models hurts the latency of individual queries. This implies that if we explore the option of GPU partition to reduce carbon footprint, this will inevitably violate the service level agreement (SLA) due to the latency increase. However, recall that different variants in a model family have different numbers of floating point operations during inference, hence different inference latency. If we carefully configure the model variants when partitioning the GPU, it is possible to take advantage of the reduced carbon footprint from both the mixed model variants and partitioned GPUs while meeting the SLA. 

% In our experimental setups so far, we have kept the carbon intensity constant for more accessible discussion of the trade-off among accuracy, carbon savings, and SLA. But, in practice, the carbon intensity of the energy source varies -- making the trade-off space even more challenging to exploit.  \sol{} adapts to carbon intensity change to intelligently trade-offs among accuracy, carbon footprint, and SLA. 

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{figures/motiv3_ci.pdf}    
%     \hrule
%     \vspace{-0.4cm}    
%     \caption{The carbon intensity during a 14-day span in March and September 2021 from two grid operators: California Independent System Operator (CISO) and UK Electricity System Operator (ESO).}
%     \vspace{-0.5cm}
%     \label{fig:motiv3_ci}
% \end{figure}

% \vspace{1.5mm}
% \noindent\textbf{Opportunity 3. Carbon intensity significantly varies over time during different seasons and across geographical locations. An intelligent workload scheduling must exploit these spatial and temporal opportunities to navigate the trade-off among: carbon footprint savings, accuracy and SLA. This can be achieved via dynamically adjusting the GPU partitions among co-located models and creating a mix of different quality models.} 
% \vspace{1.5mm}

% Fig.~\ref{fig:motiv3_ci} shows the carbon intensity data that we collect from real power system operators in California and the UK~\cite{us-ci, uk-ci}. We observe that the carbon intensity can vary by more than 200 $\text{gCO}_2$/kWh within half a day, indicating that a carbon-aware inference system must continuously optimize its configuration based on the carbon intensity. The presence of variation in carbon intensity across different geographical locations and during different seasons reiterates the need for a carbon-aware solution. Fig.~\ref{fig:motiv3_ci} reveals that the patterns of the variation are distinctively different between regions over time due to different availability of unpredictable renewable energy sources, so fine-tuned solutions (e.g., adjusting inference configuration based on the exact time of the day and date of the year) for a particular time period is neither future-proof and nor effective in other geographical regions. Motivated by these trends, we present the design of \sol{}, the first carbon-aware machine learning inference system.


% %----------- scratch space ----
% %\noindent\textbf{Opportunity 1. Mixing model variants of different sizes and qualities could trade minor accuracy degradation for a significant reduction in the carbon footprint.} 
% %\noindent\textbf{Opportunity 2. Partitioning the GPU provides an opportunity to reduce the carbon footprint through more efficient usage of GPU resources, but how to exploit this opportunity is not straightforward.} 
% %\noindent\textbf{Opportunity 3. Carbon intensity  significantly varies over time during different seasons across geographical locations.} 
% %this was not flowing.
% %This may not be interesting when the carbon intensity is constant, because one can simply pick the highest accuracy combination while limiting the carbon footprint under a target threshold (e.g., 50\% of the carbon footprint using the highest quality models). However, when the carbon intensity varies (e.g., from 500 $\text{gCO}_2$/kWh to 50 $\text{gCO}_2$/kWh), for every kWh, 50\% of carbon reduction means reducing 250 $\text{gCO}_2$ emissions with carbon intensity = 500 $\text{gCO}_2$/kWh while only reducing 25 $\text{gCO}_2$ with carbon intensity = 50 $\text{gCO}_2$/kWh, hence the same amount of accuracy degradation may not be worthy for only 25 $\text{gCO}_2$ per kWh any more after the carbon intensity drops. Therefore, a carbon-aware inference system should be able to balance the trade-off between accuracy and carbon footprint reduction in a dynamic environment.


